Simulating hard photon production with WHIZARD

One of the important goals of the proposed future $e^+e^-$ collider experiments is the search for dark matter particles using different experimental approaches. The most general search approach is based on the mono-photon signature, which is expected when production of the invisible final state is accompanied by a hard photon from initial state radiation. Analysis of the energy spectrum and angular distributions of those photons can shed light on the nature of dark matter and its interactions. Therefore, it is crucial to be able to simulate the signal and background samples in a uniform framework, to avoid possible systematic biases. The WHIZARD program is a flexible tool, which is widely used by $e^+e^-$ collaborations for simulation of many different "new physics" scenarios. We propose the procedure of merging the matrix element calculations with the lepton ISR structure function implemented in WHIZARD. It allows us to reliably simulate the mono-photon events, including the two main Standard Model background processes: radiative neutrino pair production and radiative Bhabha scattering. We demonstrate that cross sections and kinematic distributions of mono-photon in neutrino pair-production events agree with corresponding predictions of the KKMC, a Monte Carlo generator providing perturbative predictions for SM and QED processes, which has been widely used in the analysis of LEP data.

==> tex/bha_tab_Escan.tex <==
  \begin{tabular}{||c|c|c|c|c||}
    \hline
    \multirow{2}{4em}{$\sqrt{s} [GeV]$} &
	  \multicolumn{3}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma)$ [fb]} &
	  \multirow{2}{12em}{$\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma))$ [fb] after ISR rejection} \\
    & $\Pep\Pem+\gamma_{ME}$ &  $\Pep\Pem+2\gamma_{ME}$ & $\Pep\Pem+3\gamma_{ME}$ &\\
    \hline
    240 &  2.3E+05 & 2.5E+04 & 4.8E+02 & 2.2E+05\\
    250 & 2.2E+05  & 2.5E+04 & 7.3E+02 & 2.1E+05 \\
    380 & 1.4E+05 &  1.7E+04 &  5.4E+02 & 1.3E+05\\
    500 & 9.9E+04 & 1.4E+04 & 3.3E+02 & 8.9E+04\\
   1000 & 3.9E+04 & 7.2E+03  & 2.7E+02 & 3.4E+04\\
   1500 & 2.3E+04 & 4.7E+03 & 1.4E+02  & 1.9E+04\\
   3000 & 8.8E+03 & 2.7E+03 & 3.3E+01 & 7.0E+03\\
    \hline
\end{tabular}


==> tex/bha_tab_qscan.tex <==
  \begin{tabular}{||c|c|c|c|c|c||}
    \hline
    \multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} &
	  \multicolumn{3}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma)$ [fb]} &
    \multirow{2}{12em}{$\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma))$ after ISR selection} \\
    & & $\Pep\Pem+\gamma_{ME}$ &  $\Pep\Pem+2\gamma_{ME}$ & $\Pep\Pem+3\gamma_{ME}$ &\\
    \hline
    \multirow{3}{4em}{380}& $q_{min}$=1  &  1.4E+05  &  1.7E+04 &  5.4E+02  & 1.3E+05  \\
                          & $q_{min}$=5  &  1.4E+05  &  9.2E+03 & 3.1E+02  & 1.3E+05 \\
                          & $q_{min}$=10 &  1.4E+05  &  4.9E+03 & 1.4E+02  & 1.3E+05 \\
                          & $q_{min}$=50 &  1.1E+04   & 1.5E+02 & 1.8E+00  & 1.1E+04\\
    \hline
    \multirow{3}{4em}{3000}& $q_{min}$=1  & 8.8E+03   & 2.7E+03 & 3.3E+01  & 7.0E+03 \\
                           & $q_{min}$=5  &  8.9E+03  & 1.8E+03 & 3.0E+01  & 7.5E+04\\
                           & $q_{min}$=10  & 8.8E+03   & 1.2E+03 & 2.2E+01   & 7.3E+04 \\
                           & $q_{min}$=50  & 6.9E+03   &  2.8E+02 & 7.4E+00  & 6.0E+03\\
    \hline
\end{tabular}


==> tex/tab_4gm_bhabha_hard.tex <==
\begin{tabular}{||c|c|c|c|c|c|c||}
\hline
\multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} & 
\multicolumn{4}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma)$ } & 
\multirow{2}{12em}{$\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma))$ after ISR selection} \\ 
& & $\Pep\Pem+\gamma_{ME}$ &  $\Pep\Pem+2\gamma_{ME}$ & $\Pep\Pem+3\gamma_{ME}$ &  $\Pep\Pem+4\gamma_{ME}$ &\\ 
\hline
\multirow{3}{4em}{380} 
& noISR+noBS& 128100  \iffalse 128069.61 +- 223.0 \fi & 16700  \iffalse 16713.624 +- 147.0 \fi & 1100  \iffalse 1095.2868 +- 64.7 \fi & 2  \iffalse 2.0985205 +- 0.372 \fi & 145900  \iffalse 145880.62*1.0 +- 275.0 \fi \\ 
& BS& 407600  \iffalse 407564.14 +- 923.0 \fi & 29600  \iffalse 29633.157 +- 267.0 \fi & 640  \iffalse 638.70111 +- 41.8 \fi & 4  \iffalse 4.260272 +- 0.702 \fi & 437800  \iffalse 437840.26*1.0 +- 962.0 \fi \\ 
& ISR& 139200  \iffalse 139204.91 +- 318.0 \fi & 17600  \iffalse 17625.001 +- 230.0 \fi & 520  \iffalse 522.50027 +- 35.9 \fi & 3  \iffalse 2.6764745 +- 0.548 \fi & 125100  \iffalse 157355.09*0.79485 +- 394.0 \fi \\ 
& BS+ISR& 144900  \iffalse 144886.92 +- 338.0 \fi & 18200  \iffalse 18244.667 +- 177.0 \fi & 530  \iffalse 533.58575 +- 25.3 \fi & 0  \iffalse 0.077953483 +- 0.0396 \fi & 131700  \iffalse 163665.25*0.8046 +- 382.0 \fi \\ 
\hline 
\multirow{3}{4em}{3000} 
& noISR+noBS& 5800  \iffalse 5799.5094 +- 13.1 \fi & 2200  \iffalse 2210.6642 +- 19.6 \fi & 77  \iffalse 77.229792 +- 3.66 \fi & 0  \iffalse 0.38370555 +- 0.106 \fi & 8100  \iffalse 8087.7872*1.0 +- 23.8 \fi \\ 
& BS& 221600  \iffalse 221621.77 +- 2330.0 \fi & 15100  \iffalse 15104.727 +- 454.0 \fi & 88  \iffalse 87.712368 +- 6.84 \fi & 2  \iffalse 1.7405703 +- 0.411 \fi & 236800  \iffalse 236815.95*1.0 +- 2380.0 \fi \\ 
& ISR& 8900  \iffalse 8859.4014 +- 37.4 \fi & 2500  \iffalse 2545.371 +- 40.8 \fi & 74  \iffalse 74.182503 +- 5.54 \fi & 0  \iffalse 0.06025432 +- 0.014 \fi & 6900  \iffalse 11479.015*0.6047 +- 55.6 \fi \\ 
& BS+ISR& 20400  \iffalse 20365.013 +- 220.0 \fi & 3800  \iffalse 3822.0738 +- 137.0 \fi & 100  \iffalse 103.04921 +- 9.84 \fi & 0  \iffalse 0.18778198 +- 0.0361 \fi & 15900  \iffalse 24290.324*0.6532 +- 260.0 \fi \\ 
\hline 
\end{tabular} 


==> tex/tab_4gm_vv_hard.tex <==
\begin{tabular}{||c|c|c|c|c|c|c||}
\hline
\multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} &
\multicolumn{4}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
\multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after ISR selection} \\ 
& &  $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ & $\PGn\PAGn+3\gamma_{ME}$ & $\PGn\PAGn+4\gamma_{ME}$ &\\ 
\hline
\multirow{3}{4em}{380} 
& noISR+noBS& 3000  \iffalse 3008.1674 +- 3.88 \fi & 550  \iffalse 553.50007 +- 1.47 \fi & 48  \iffalse 48.396165 +- 1.76 \fi & 1  \iffalse 0.60103864 +- 0.0465 \fi & 3600  \iffalse 3610.6647*1.0 +- 4.51 \fi \\ 
& BS& 3000  \iffalse 3032.9037 +- 3.74 \fi & 560  \iffalse 559.07522 +- 1.4 \fi & 45  \iffalse 44.528861 +- 1.24 \fi & 1  \iffalse 0.60310017 +- 0.0557 \fi & 3600  \iffalse 3637.1109*1.0 +- 4.18 \fi \\ 
& ISR& 3200  \iffalse 3160.0878 +- 4.0 \fi & 570  \iffalse 572.01033 +- 1.55 \fi & 48  \iffalse 47.587295 +- 1.8 \fi & 0  \iffalse 0.28838589 +- 0.0328 \fi & 3100  \iffalse 3779.9738*0.8077 +- 4.65 \fi \\ 
& BS+ISR& 3200  \iffalse 3201.2746 +- 4.19 \fi & 580  \iffalse 576.79445 +- 1.54 \fi & 43  \iffalse 42.583633 +- 2.03 \fi & 2  \iffalse 1.5346674 +- 0.127 \fi & 3100  \iffalse 3822.1873*0.8112 +- 4.91 \fi \\ 
\hline 
\multirow{3}{4em}{3000} 
& noISR+noBS& 4300  \iffalse 4281.0649 +- 8.01 \fi & 1300  \iffalse 1299.0039 +- 6.78 \fi & 150  \iffalse 150.87037 +- 7.16 \fi & 4  \iffalse 3.7178354 +- 0.528 \fi & 5700  \iffalse 5734.657*1.0 +- 12.7 \fi \\ 
& BS& 4100  \iffalse 4103.3137 +- 8.08 \fi & 1200  \iffalse 1204.9407 +- 7.23 \fi & 130  \iffalse 131.27277 +- 8.07 \fi & 1  \iffalse 1.0127015 +- 0.144 \fi & 5400  \iffalse 5440.5399*1.0 +- 13.5 \fi \\ 
& ISR& 4200  \iffalse 4200.6125 +- 7.86 \fi & 1300  \iffalse 1260.2989 +- 7.28 \fi & 140  \iffalse 143.7677 +- 13.3 \fi & 2  \iffalse 1.9109029 +- 0.231 \fi & 3900  \iffalse 5606.59*0.69365 +- 17.1 \fi \\ 
& BS+ISR& 4000  \iffalse 4036.2122 +- 8.32 \fi & 1200  \iffalse 1183.2086 +- 7.42 \fi & 130  \iffalse 134.01589 +- 7.28 \fi & 1  \iffalse 0.72332279 +- 0.0899 \fi & 3800  \iffalse 5354.16*0.70155 +- 13.3 \fi \\ 
\hline 
\end{tabular} 


==> tex/tab_4gm_vv_hard_corr.tex <==
\begin{tabular}{||c|c|c|c|c|c|c||}
\hline
\multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} &
\multicolumn{4}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
\multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after ISR selection} \\ 
& &  $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ & $\PGn\PAGn+3\gamma_{ME}$ & $\PGn\PAGn+4\gamma_{ME}$ &\\ 
\hline
\multirow{3}{4em}{380} 
& noISR+noBS& 3000  \iffalse 3008.1362 +- 3.94 \fi & 1800  \iffalse 1752.8897 +- 4.08 \fi & 480  \iffalse 483.43831 +- 10.4 \fi & 38  \iffalse 37.980948 +- 3.4 \fi & 5300  \iffalse 5282.4451*1.0 +- 12.3 \fi \\ 
& BS& 3000  \iffalse 3030.6864 +- 3.74 \fi & 1600  \iffalse 1580.9689 +- 3.6 \fi & 370  \iffalse 366.32003 +- 7.82 \fi & 32  \iffalse 32.189263 +- 2.21 \fi & 5000  \iffalse 5010.1647*1.0 +- 9.64 \fi \\ 
& ISR& 3200  \iffalse 3160.0878 +- 4.0 \fi & 570  \iffalse 572.01033 +- 1.55 \fi & 48  \iffalse 47.587295 +- 1.8 \fi & 0  \iffalse 0.28838589 +- 0.0328 \fi & 3100  \iffalse 3779.9738*0.8077 +- 4.65 \fi \\ 
& BS+ISR& 3200  \iffalse 3201.2746 +- 4.19 \fi & 580  \iffalse 576.79445 +- 1.54 \fi & 43  \iffalse 42.583633 +- 2.03 \fi & 2  \iffalse 1.5346674 +- 0.127 \fi & 3100  \iffalse 3822.1873*0.8112 +- 4.91 \fi \\ 
\hline 
\multirow{3}{4em}{3000} 
& noISR+noBS& 4300  \iffalse 4266.6092 +- 7.48 \fi & 3700  \iffalse 3703.5207 +- 16.0 \fi & 1600  \iffalse 1610.6853 +- 14.5 \fi & 160  \iffalse 156.03754 +- 9.35 \fi & 9700  \iffalse 9736.8527*1.0 +- 24.7 \fi \\ 
& BS& 4100  \iffalse 4111.7548 +- 8.37 \fi & 2900  \iffalse 2945.2319 +- 15.2 \fi & 1100  \iffalse 1068.6627 +- 15.7 \fi & 46  \iffalse 46.009218 +- 5.45 \fi & 8200  \iffalse 8171.6586*1.0 +- 24.0 \fi \\ 
& ISR& 4200  \iffalse 4200.6125 +- 7.86 \fi & 1300  \iffalse 1260.2989 +- 7.28 \fi & 140  \iffalse 143.7677 +- 13.3 \fi & 2  \iffalse 1.9109029 +- 0.231 \fi & 3900  \iffalse 5606.59*0.69365 +- 17.1 \fi \\ 
& BS+ISR& 4000  \iffalse 4036.2122 +- 8.32 \fi & 1200  \iffalse 1183.2086 +- 7.42 \fi & 130  \iffalse 134.01589 +- 7.28 \fi & 1  \iffalse 0.72332279 +- 0.0899 \fi & 3800  \iffalse 5354.16*0.70155 +- 13.3 \fi \\ 
\hline 
\end{tabular} 


==> tex/tab_qscan_bhabha_hard_4gm.tex <==
\begin{tabular}{||c|c|c|c|c|c||}
\hline
\multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} & 
\multicolumn{3}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma)$ } & 
\multirow{2}{12em}{$\sigma(\Pep\Pem\rightarrow\Pep\Pem+N\gamma))$ after ISR selection} \\ 
& & $\Pep\Pem+\gamma_{ME}$ &  $\Pep\Pem+2\gamma_{ME}$ & $\Pep\Pem+3\gamma_{ME}$ & \\ 
\hline
\multirow{3}{4em}{380} 
& noISR+noBS& 128100  \iffalse 128069.61 +- 223.0 \fi & 16700  \iffalse 16713.624 +- 147.0 \fi & 1100  \iffalse 1095.2868 +- 64.7 \fi & 0  \iffalse 2.0985205*0.0 +- 0.372 \fi \\ 
& BS& 407600  \iffalse 407564.14 +- 923.0 \fi & 29600  \iffalse 29633.157 +- 267.0 \fi & 640  \iffalse 638.70111 +- 41.8 \fi & 0  \iffalse 4.260272*0.0 +- 0.702 \fi \\ 
& ISR& 139200  \iffalse 139204.91 +- 318.0 \fi & 17600  \iffalse 17625.001 +- 230.0 \fi & 520  \iffalse 522.50027 +- 35.9 \fi & 0  \iffalse 2.6764745*0.0 +- 0.548 \fi \\ 
& BS+ISR& 144900  \iffalse 144886.92 +- 338.0 \fi & 18200  \iffalse 18244.667 +- 177.0 \fi & 530  \iffalse 533.58575 +- 25.3 \fi & 0  \iffalse 0.077953483*0.0 +- 0.0396 \fi \\ 
\hline 
\multirow{3}{4em}{3000} 
& noISR+noBS& 5800  \iffalse 5799.5094 +- 13.1 \fi & 2200  \iffalse 2210.6642 +- 19.6 \fi & 77  \iffalse 77.229792 +- 3.66 \fi & 0  \iffalse 0.38370555*0.0 +- 0.106 \fi \\ 
& BS& 221600  \iffalse 221621.77 +- 2330.0 \fi & 15100  \iffalse 15104.727 +- 454.0 \fi & 88  \iffalse 87.712368 +- 6.84 \fi & 0  \iffalse 1.7405703*0.0 +- 0.411 \fi \\ 
& ISR& 8900  \iffalse 8859.4014 +- 37.4 \fi & 2500  \iffalse 2545.371 +- 40.8 \fi & 74  \iffalse 74.182503 +- 5.54 \fi & 0  \iffalse 0.06025432*0.0 +- 0.014 \fi \\ 
& BS+ISR& 20400  \iffalse 20365.013 +- 220.0 \fi & 3800  \iffalse 3822.0738 +- 137.0 \fi & 100  \iffalse 103.04921 +- 9.84 \fi & 0  \iffalse 0.18778198*0.0 +- 0.0361 \fi \\ 
\hline 
\end{tabular} 


==> tex/tab_qscan_vv_hard_4gm.tex <==
\begin{tabular}{||c|c|c|c|c|c||}
\hline
\multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} &
\multicolumn{3}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
\multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after ISR selection} \\ 
& &  $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ & $\PGn\PAGn+3\gamma_{ME}$ &\\ 
\hline
\multirow{3}{4em}{380} 
& noISR+noBS& 3000  \iffalse 3008.1674 +- 3.88 \fi & 550  \iffalse 553.50007 +- 1.47 \fi & 48  \iffalse 48.396165 +- 1.76 \fi & 0  \iffalse 0.60103864*0.0 +- 0.0465 \fi \\ 
& BS& 3000  \iffalse 3032.9037 +- 3.74 \fi & 560  \iffalse 559.07522 +- 1.4 \fi & 45  \iffalse 44.528861 +- 1.24 \fi & 0  \iffalse 0.60310017*0.0 +- 0.0557 \fi \\ 
& ISR& 3200  \iffalse 3160.0878 +- 4.0 \fi & 570  \iffalse 572.01033 +- 1.55 \fi & 48  \iffalse 47.587295 +- 1.8 \fi & 0  \iffalse 0.28838589*0.0 +- 0.0328 \fi \\ 
& BS+ISR& 3200  \iffalse 3201.2746 +- 4.19 \fi & 580  \iffalse 576.79445 +- 1.54 \fi & 43  \iffalse 42.583633 +- 2.03 \fi & 0  \iffalse 1.5346674*0.0 +- 0.127 \fi \\ 
\hline 
\multirow{3}{4em}{3000} 
& noISR+noBS& 4300  \iffalse 4281.0649 +- 8.01 \fi & 1300  \iffalse 1299.0039 +- 6.78 \fi & 150  \iffalse 150.87037 +- 7.16 \fi & 0  \iffalse 3.7178354*0.0 +- 0.528 \fi \\ 
& BS& 4100  \iffalse 4103.3137 +- 8.08 \fi & 1200  \iffalse 1204.9407 +- 7.23 \fi & 130  \iffalse 131.27277 +- 8.07 \fi & 0  \iffalse 1.0127015*0.0 +- 0.144 \fi \\ 
& ISR& 4200  \iffalse 4200.6125 +- 7.86 \fi & 1300  \iffalse 1260.2989 +- 7.28 \fi & 140  \iffalse 143.7677 +- 13.3 \fi & 0  \iffalse 1.9109029*0.0 +- 0.231 \fi \\ 
& BS+ISR& 4000  \iffalse 4036.2122 +- 8.32 \fi & 1200  \iffalse 1183.2086 +- 7.42 \fi & 130  \iffalse 134.01589 +- 7.28 \fi & 0  \iffalse 0.72332279*0.0 +- 0.0899 \fi \\ 
\hline 
\end{tabular} 


==> tex/vv_tab1.tex <==
  
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \multirow{2}{4em}{$\sqrt{s}[GeV]$} &
    \multicolumn{4}{|c|}{ Whizard-2.8
      $\sigma(\Pep\Pem\rightarrow\nu\bar{\nu})$ } &
    \multirow{2}{4em}{$\sigma(\Pep\Pem\rightarrow\nu\bar{\nu})$ after
      ISR selection} \\
    & $\nu\bar{\nu}$ &  $\nu\bar{\nu}+\gamma_{ME}$ &  $\nu\bar{\nu}+2\gamma_{ME}$ &
    $\nu\bar{\nu}+3\gamma_{ME}$ & \\
    240 &5.3946391E+04  $\pm$1.23E+01 & 1.2598297E+04 $\pm$1.12E+01 &
    1.3388854E+03 $\pm$2.13E+00  &
    7.8500540E+01 $\pm$2.60E+00 & 6.7962073E+04*eff $\pm$1.70E+01\\
    250 & 5.3250418E+04 $\pm$1.41E+01 & 1.2257647E+04 $\pm$1.12E+01 &
    1.2939339E+03 $\pm$ 1.92E+00 &
    7.5266145E+01 $\pm$ 2.03E+00 & 6.6877266E+04*eff $\pm$1.82E+01\\
    380 & 5.0860906E+04 $\pm$1.16E+01 & 1.0932619E+04 $\pm$9.99E+00 &
    1.1607523E+03 $\pm$2.20E+00  &
    7.3812969E+01 $\pm$ 2.06E+00 & 6.3028090E+04*eff $\pm$1.56E+01\\
    500 & 5.1165563E+04 $\pm$ 1.33E+01 & 1.1278812E+04 $\pm$1.06E+01 &
    1.2330646E+03 $\pm$2.19E+00  &
    6.0991918E+01 $\pm$1.96E+00 & 6.3738431E+04*eff $\pm$1.73E+01\\
    1000 & 5.2737274E+04 $\pm$9.79E+00 & 1.3648468E+04 $\pm$1.36E+01 &
    1.7459249E+03 $\pm$4.10E+00  &
    1.3607508E+02 $\pm$2.65E+00  & 6.8267742E+04*eff $\pm$1.74E+01\\
    1500 & 5.3376531E+04 $\pm$1.43E+01 & 1.5359572E+04 $\pm$1.58E+01 &
    2.1733894E+03 $\pm$ 5.53E+00 &
    1.9410857E+02 $\pm$ 4.72E+00 & 7.1103600E+04*eff $\pm$2.25E+01\\
    3000 & 5.3918791E+04 $\pm$ 1.60E+01 & 1.8420638E+04 $\pm$ 1.93E+01
    & 3.1445354E+03 $\pm$1.08E+01 &
    2.8501502E+02 $\pm$1.70E+01  & 7.5768980E+04*eff $\pm$3.22E+01\\
    \hline
\end{tabular}


==> tex/vv_tab_Escan.tex <==
  \begin{tabular}{||c|c|c|c|c|c||}
    \hline
    \multirow{2}{4em}{$\sqrt{s}[GeV]$} &
    \multicolumn{4}{|c|}{ Whizard-2.8
      $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
    \multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after
      ISR selection} \\
    & $\PGn\PAGn$ &  $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ &
    $\PGn\PAGn+3\gamma_{ME}$ & \\
    \hline
    240 & 5.4E+04 & 1.3E+04 & 1.3E+03 & 6.3E+02 & 5.4E+04 \\
    250 & 5.3E+04 & 1.2E+04 & 1.3E+03 & 6.0E+02 & 5.3E+04 \\
    380 & 5.1E+04 & 1.1E+04 & 1.2E+03 & 5.5E+02 & 5.1E+04 \\
    500 & 5.1E+04 & 1.1E+04 & 1.2E+03 & 7.5E+02 & 5.1E+04 \\
    1000 & 5.3E+04 & 1.4E+04 & 1.7E+03 & 1.2E+03 & 5.2E+04 \\
    1500 & 5.3E+04 & 1.5E+04 & 2.2E+03 & 1.7E+03 & 5.2E+04 \\
    3000 & 5.4E+04 & 1.8E+04 & 3.1E+03 & 1.8E+03 & 5.2E+04 \\
    \hline
\end{tabular}


==> tex/vv_tab_hard.tex <==
  \begin{tabular}{||c|c|c|c|c||}
    \hline
    \multirow{2}{4em}{$\sqrt{s}[GeV]$} &
    \multicolumn{3}{c|}{ Whizard-2.8
      $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
    \multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after
      ISR selection} \\
    &  $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ &    $\PGn\PAGn+3\gamma_{ME}$ & \\
    \hline
    240  & 4.2E+03 &  7.3E+02 & 3.7E+01 & 3.2E+03 \\
    250  & 4.1E+03 &  6.9E+02 & 4.8E+01 & 3.9E+03\\
    380  & 4.3E+03 &  1.4E+03 & 1.3E+02 & 3.9E+03 \\
    500  & 3.1E+03 &  5.9E+02 & 4.8E+01 & 3.0E+03\\
    1000 & 3.5E+03 & 7.8E+02 & 7.4E+01 & 3.3E+03 \\
    1500 & 3.8E+03 & 9.4E+02 & 9.8E+01 & 3.6E+03\\
    3000 & 4.2E+03 & 1.3E+03 & 1.4E+02 & 3.9E+03 \\
    \hline
\end{tabular}


==> tex/vv_tab_qscan.tex <==
  \begin{tabular}{||c|c|c|c|c|c|c||}
    \hline
    \multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} &
    \multicolumn{4}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
    \multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after ISR selection} \\
    & & $\PGn\PAGn$ &  $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ & $\PGn\PAGn+3\gamma_{ME}$ &\\
    \hline
    \multirow{3}{4em}{380} & $q_{min}$=1   & 5.1E+04 & 1.1E+04 & 1.2E+03 &  5.5E+02 & 5.1E+04 \\
                           & $q_{min}$=5   & 5.1E+04 & 7.0E+03 & 4.8E+02 &  1.5E+01 & 5.1E+04 \\
                           & $q_{min}$=10  & 5.1E+04 & 5.3E+03 & 2.8E+02 &  8E+01 & 5.1E+04 \\
                           & $q_{min}$=50  & 5.1E+04 & 1.4E+03 & 2.2E+01 &   1E-01 &  5.1E+04 \\
    \hline
    \multirow{3}{4em}{3000} & $q_{min}$=1   & 5.4E+04  & 1.8E+04 & 3.1E+03 & 1.8E+03 & 5.2E+04 \\
                            & $q_{min}$=5   & 5.4E+04  & 1.3E+04 & 1.6E+03 & 7.4E+01 & 5.3E+04 \\
                            & $q_{min}$=10  & 5.4E+04 & 1.1E+04  &  1.1E+03 & 5.7E+01 & 5.3E+04 \\
                            & $q_{min}$=50  & 5.4E+04 & 5.2E+03  &  2.6E+02 & 2E+00 & 5.3E+04 \\
    \hline
\end{tabular}


==> tex/vv_tab_qscan_3TeV.tex <==
  \begin{tabular}{||c|c|c|c|c|c|c||}
    \hline
    \multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} &
    \multicolumn{4}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
    \multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after ISR selection} \\
    & & $\PGn\PAGn$ &  $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ & $\PGn\PAGn+3\gamma_{ME}$ &\\
    \hline
    \multirow{3}{4em}{380}& q=1  &  & & &  &  \\
    & q=5  &  & & &  &  \\
    & q=10  &  & & &  &  \\
    & q=50  &  & & &  &  \\
    \hline
    \multirow{3}{4em}{3000}& q=1  &  & & &  &  \\
    & q=5  &  & & &  &  \\
    & q=10  &  & & &  &  \\
    & q=50  &  & & &  &  \\
    \hline
\end{tabular}


==> tex/vv_tab_qscan_hard.tex <==
  \begin{tabular}{||c|c|c|c|c|c||}
    \hline
    \multirow{2}{4em}{$\sqrt{s} [GeV]$} & \multirow{2}{4em}{$q_{min}[GeV]$} &
    \multicolumn{3}{c|}{ Whizard-2.8 $\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ } &
    \multirow{2}{8em}{$\sigma(\Pep\Pem\rightarrow\PGn\PAGn)$ after ISR selection} \\
    & & $\PGn\PAGn+\gamma_{ME}$ &  $\PGn\PAGn+2\gamma_{ME}$ & $\PGn\PAGn+3\gamma_{ME}$ &\\
    \hline
    \multirow{3}{4em}{380} & $q_{min}$=1  & 4.3E+03  & 1.4E+03 & 1.3E+02 & 3.9E+03 \\
                           & $q_{min}$=5  & 4.3E+03  & 9.4E+02 & 5.8E+01 & 4.0E+03\\
                           & $q_{min}$=10 & 4.3E+03  & 7.5E+02 & 4.7E+01 & 4.0E+03\\
                           & $q_{min}$=50 & 4.1E+03  & 2.9E+02 & 3.8E+00 & 3.9E+03\\
    \hline
    \multirow{3}{4em}{3000}& $q_{min}$=1  & 4.2E+03  & 1.3E+03 & 1.4E+02 & 3.9E+03 \\
                           & $q_{min}$=5  & 4.2E+03  & 8.5E+02 & 6.6E+01 & 3.9E+03\\
                           & $q_{min}$=10 & 4.2E+03  & 6.8+02  & 3.1E+01 & 3.9E+03\\
                           & $q_{min}$=50 & 3.9E+03  & 2.4E+02 & 2.5E+00 & 3.7E+03\\
    \hline
\end{tabular}

